Diffuse Gamma-ray Emission Around 4FGL J1626.0-4917

Extended gamma-ray sources provide significant information about particle propagation. 4FGL J1626.0-4917 was labeled as an unassociated source in 4FGL catalog without known counterparts at other wavelengths. We report an analysis on 4FGL J1626.0-4917 with 17 years Fermi Large Area Telescope data and archival Chandra X-ray Observatory data. We find extended GeV emission around this source, which can be modelled by a Gaussian disk of 0.28 degree radius with a significance of the extension of 7.2 sigma. The gamma-ray spectrum of 4FGL J1626.0-4917 has a photon index of 2.73. The gas content, including molecular, neutral and ionized gas, was investigated and the potential hadronic origin is discussed. The diffuse GeV gamma-ray emission may likely originate from the interaction between accelerated protons in 4FGL J1626.0-4917 and the target proton in surrounding gas, although the leptonic process cannot be ruled out. The X-ray spectral analysis was performed, which reveal a point source inside 4FGL J1626.0-4917. We investigate potential counterparts, including the stellar cluster NGC 6134 and the supernova remnant G335.2+0.1. Our results highlight the complexity of unidentified extended gamma-ray sources and the need for further observations.

==> readme <==
Dear Colleagues: 

The final publication layout will be produced by using raa.cls. 
Therefore, we strongly encourage you to prepare your LaTeX manuscript 
with this class file. Please unpack raa-package.tar.gz, it includes 

raa.cls        ---- RAA macro class file for LaTeX2e 
sample.tex     ---- a sample file using raa.cls (LaTeX source) 
sample.ps      ---- the PS file created by sample.tex in referee format  
sample.pdf     ---- the PDF file created by sample.tex in referee format  
readme         ---- this file  
f?.eps         ---- three demo figures used in the LaTeX template source
sample2.tex    ---- a sample file for using raa.bst
sample2_fig?.eps -- two demo figures used in sample2.tex
sample2.pdf    ---- the PDF file created by sample.tex in referee format
sample2.bbl    ---- bibliography file using by sample2.tex
bibtex.bib     ---- an example for bibtex file

natbib.sty     ---- This package reimplements the LaTeX \cite command
natnotes.pdf   ---- Brief reference sheet for Natbib (pdf)
raa.bst        ---- Bibliography style file 

Hope you enjoy the use of this macro. Your suggestions and comments are 
highly welcome. Thanks.

Editorial Office
E-mail:  raa@raa-journal.org

